Simulation Assessment Guidelines towards Independent Safety Assurance of Autonomous Vehicles

This Simulation Assessment Guidelines document is a public guidelines document developed by the Centre of Excellence for Testing & Research of AVs - NTU (CETRAN) in collaboration with the Land Transport Authority (LTA) of Singapore. It is primarily intended to help the developers of Autonomous Vehicles (AVs) in Singapore to prepare their software simulations and provide recommendations that can ensure their readiness for independent assessment of their virtual simulation results according to the Milestone-testing framework adopted by the assessor and the local authority in Singapore, namely, CETRAN and LTA respectively.

==> sections/ScenariosList.tex <==
\renewcommand{\labelenumi}{\texttt{[\arabic{enumi}]} }

\section{Reference list of test cases selected for M2 assessment}

Note that this list of test cases is only indicative and provided for an initial reference.
The actual and final set of test cases applicable to the VUT to be assessed (which may be significantly different from what is stated in the below list), will be provided separately only after the M2 application process is completed, and the simulation assessment readiness has been demonstrated through the results for the sample test case(s) provided.

\begin{itemize}
	\item \texttt{[M2-CL4-S-TST-02]} Test for Left turn slip road (with Zebra crossing)
	\begin{enumerate}
		\item No VRU/TSV
		\item TSV going straight in major road, no VRU
		\item VRU crossing, no TSV; VRU Crossing at the edge of pedestrian
		crossing, no TSV; VRU Crossing at the middle of pedestrian
		crossing, no TSV; VRU stationary at the edge of pedestrian
		crossing, no TSV
		\item Following TSV, no VRU
		\item VRU crossing and TSV in front
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-03]} Right turn at traffic light intersection
	\begin{enumerate}
		\item No VRU/TSV
		\item VRU Crossing at the Edge of Pedestrian crossing; VRU Crossing at the Middle of Pedestrian crossing
		\item Oncoming TSV from the opposite side of intersection
		\item Right turn at signalized junction - Giving way to oncoming TSV and to ap pedestrian crossing
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-04]} Test for Raised zebra crossing
	\begin{enumerate}
		\item No VRU/TSV
		\item VRU crossing, no TSV; VRU Crossing at the edge of pedestrian crossing, no TSV; VRU Crossing at the middle of pedestrian crossing, no TSV; VRU stationary at the edge of pedestrian crossing, no TSV
		\item Running VRU crossing, no TSV
		\item VRU crossing, TSV in front
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-05]} Test for overtaking stopped vehicle
	\begin{enumerate}
		\item No VRU, no oncoming TSV
		\item VRU (jaywalker) crossing after stopped vehicle
		\item No VRU, oncoming TSV
		\item VRU crossing (jay-walking) after stopped vehicle, oncoming TSV
		\item Overtaking multiple stationary cars
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-06]} Test for overtaking cyclist
	\begin{enumerate}
		\item Cyclist goes straight at constant speed
		\item Cyclist changes lane in front of VUT
		\item Cyclist swerves 1m around a small object in front of VUT, return to original lane
		\item Cyclist changes speed in front of VUT
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-07]} Signalized intersection (traffic light)
	\begin{enumerate}
		\item Solid green and turn green
		\item Solid red and turn green
		\item Changing of arrow signal from turn red to turn green
		\item Making u-turn at the junction
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-08]} Object on the Road
	\begin{enumerate}
		\item Object on the road
		\item Construction site
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-09]} Left turn at intersections
	\begin{enumerate}
		\item No Obstacle
		\item Pedestrian Crossing - from the edge; Pedestrian Crossing - from the middle
		\item Static VRU (cyclist) beside VUT; in the left side (nearside) and middle of road
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-11]} Yellow box at traffic intersection
	\begin{enumerate}
		\item No VRU, No TSV
		\item Stationary TSVs
		\item Moving TSVs
	\end{enumerate}
	\item \texttt{[M2-CL4-S-TST-14]} Tests for virtual vehicle dynamics fidelity check
	\begin{enumerate}
		\item Acceleration test
		\item Braking test
		\item Coast down test
	\end{enumerate}
\end{itemize}

\renewcommand{\labelenumi}{\arabic{enumi}. }


==> sections/report_generation.tex <==
\newpage

\section{Report generation}


After the virtual testing and assessment is completed, a report shall be generated by CETRAN and submitted to LTA. 
LTA will review CETRAN's recommendations and make the final decision on M2 assessment outcome.

The final report will include:
\begin{itemize}
	\item Details of VUT ADS software and hardware (if any) under test, including version numbers.	
	\item Strengths and gaps of the Virtual Testing Toolchain of the AV developer as stated by the AV developer	
	\item CETRAN's observations about the Virtual Testing Toolchain of the AV developer	
	\item Plots of interesting parameters from the simulation results, for each test case
	\item Fidelity check of simulation results
	\item Evaluation of simulation results based on KPI values, for each test case
	\item Final recommendation (pass/fail/others)
\end{itemize}



\begin{table}[h]
	\setlength\nwidth{5.5em}    %% minimum block width
	\setlength\nheight{6em}     %% minimum block height
	\centering
	\caption{Final simulation assessment report}
	\label{tab:Repot}
	\begin{tabular}{>{\centering}m{\nwidth}m{50mm}m{\textwidth - 50mm - \nwidth - 6\tabcolsep}}
		\hline\hline
		\textbf{Topic} & \textbf{Output} & \textbf{Remarks}\tabularnewline
		\hline\smallskip
		\tikz{\node[block] {\includegraphics[width=3.5em]{scenario_verification.png}\\Final report};}
		& Final recommendation based on assessed results 
		& Pass/fail recommendation together with justification \tabularnewline
		\hline\hline
	\end{tabular}
\end{table}

==> sections/timelines.tex <==
\newpage

\section{Testing timeline}

To ensure a smooth and efficient assessment, we propose certain timelines that have to be respected. In particular:

\begin{itemize}
	\item AV developer to acknowledge receipt of the `simulation scenarios package' within 3 working days of receiving it
	\item AV developer to complete all simulations and submit the results (along with any qualitative remarks, screenshots, other supplementary material etc.) within 7 working days.
	
\end{itemize}

Please note that these timelines are subject to further optimization; they could be fine-tuned through mutual discussions and in smooth coordination with other related processes for M2 assessment, such as a pre-check, physical testing and document review as applicable.


\begin{figure}[h]
	\centering
	\vspace{1ex}
	\includegraphics[width=\textwidth]{figures/timelines}
	\caption{Timelines to be followed during the Virtual Testing Process}
	\label{fig:timelines}
\end{figure}

